Multi-Scale Graph Learning for Anti-Sparse Downscaling

Water temperature can vary substantially even across short distances within the same sub-watershed. Accurate prediction of stream water temperature at fine spatial resolutions (i.e., fine scales, $\leq$ 1 km) enables precise interventions to maintain water quality and protect aquatic habitats. Although spatiotemporal models have made substantial progress in spatially coarse time series modeling, challenges persist in predicting at fine spatial scales due to the lack of data at that scale.To address the problem of insufficient fine-scale data, we propose a Multi-Scale Graph Learning (MSGL) method. This method employs a multi-task learning framework where coarse-scale graph learning, bolstered by larger datasets, simultaneously enhances fine-scale graph learning. Although existing multi-scale or multi-resolution methods integrate data from different spatial scales, they often overlook the spatial correspondences across graph structures at various scales. To address this, our MSGL introduces an additional learning task, cross-scale interpolation learning, which leverages the hydrological connectedness of stream locations across coarse- and fine-scale graphs to establish cross-scale connections, thereby enhancing overall model performance. Furthermore, we have broken free from the mindset that multi-scale learning is limited to synchronous training by proposing an Asynchronous Multi-Scale Graph Learning method (ASYNC-MSGL). Extensive experiments demonstrate the state-of-the-art performance of our method for anti-sparse downscaling of daily stream temperatures in the Delaware River Basin, USA, highlighting its potential utility for water resources monitoring and management.

==> preamble_unused.tex <==


% if you need to pass options to natbib, use, e.g.:
%     \PassOptionsToPackage{numbers, compress}{natbib}
% before loading neurips_2024





% ready for submission
\usepackage{aaai25}





\usepackage[utf8]{inputenc} % allow utf-8 input
\usepackage[T1]{fontenc}    % use 8-bit T1 fonts
\usepackage{hyperref}
\usepackage{url}            % simple URL typesetting
\usepackage{booktabs}       % professional-quality tables
\usepackage{amsfonts}       % blackboard math symbols
\usepackage{nicefrac}       % compact symbols for 1/2, etc.
\usepackage{microtype}      % microtypography



\usepackage[table]{xcolor} %2024.5.7
\definecolor{lightblue}{rgb}{0.882, 0.913, 0.964}%2024.5.7
\definecolor{midblue}{rgb}{0.706, 0.792, 0.902}%2024.5.7
\definecolor{darkblue}{rgb}{0.564, 0.690, 0.850}%2024.5.7
\definecolor{lightred}{rgb}{0.984, 0.905, 0.917}%2024.5.7
\definecolor{superlightblue}{rgb}{0.878, 1.000, 1.000} %2024.5.9
\usepackage{colortbl}%2024.5.7
\usepackage{hhline}%2024.5.7


\usepackage{csquotes}
\usepackage{amsmath}
\usepackage{wrapfig}
\usepackage{graphicx}
\usepackage{thmtools}
\usepackage{thm-restate}
\usepackage{mathtools}
\usepackage{amsthm}

%\usepackage[numbers,sort]{natbib}

\input{lettres_maths.tex}
\input{theoremes.tex}
\theoremstyle{plain}

\usepackage[english]{babel}
\usepackage{comment}
\usepackage{tabularx} %2024.5.7
\usepackage{gensymb} %2024.5.9









%%%%%%%%%%%%%%%%%%%%%%
\usepackage{algorithm,algorithmicx,algpseudocode}
\usepackage{times}
\usepackage{epsfig}
\usepackage{float}
\usepackage{wrapfig}
\usepackage{amssymb}
\usepackage{bm,xspace}
\usepackage{verbatim}
\usepackage{multirow}
\usepackage{balance}
\usepackage{etoolbox,siunitx}
\usepackage{calc}
\usepackage{pifont,hologo}
\setlength\heavyrulewidth{0.10em}
\setlength\lightrulewidth{0.05em}
\setlength\cmidrulewidth{0.03em}
\newcommand{\ra}[1]{\renewcommand{\arraystretch}{#1}}
\usepackage[super]{nth}
\sisetup{detect-weight=true,detect-inline-weight=math}
\sisetup{quotient-mode = fraction}
\sisetup{fraction-function = \nicefrac}
\robustify\bfseries
\usepackage{dsfont}
\usepackage{makecell} %2024.5.17
% 补丁代码，用于移除算法编号
% 移除 algorithm 环境的编号
\makeatletter %2024.5.17
\renewcommand{\fnum@algorithm}{\fname@algorithm} %2024.5.17
\makeatother  %2024.5.17
\usepackage{relsize} %2024.5.18
\usepackage{enumitem} %2024.5.19



%\setlength{\textfloatsep}{0.1cm}
%\setlength{\intextsep}{0pt plus 2pt}
%\setlength{\floatsep}{0pt}
%\captionsetup[table]{skip=1pt}

\def\aa{\mathbf{a}}
\def\bb{\mathbf{b}}
\def\cc{\mathbf{c}}
\def\dd{\mathbf{d}}
\def\ee{\mathbf{e}}
\def\ff{\mathbf{f}}
\def\gg{\mathbf{g}}
\def\hh{\mathbf{h}}
\def\ii{\mathbf{i}}
\def\jj{\mathbf{j}}
\def\kk{\mathbf{k}}
\def\ll{\mathbf{l}}
\def\mm{\mathbf{m}}
\def\nn{\mathbf{n}}
\def\oo{\mathbf{o}}
\def\pp{\mathbf{p}}
\def\qq{\mathbf{q}}
\def\rr{\mathbf{r}}
\def\sss{\mathbf{s}}
\def\tt{\mathbf{t}}
\def\uu{\mathbf{u}}
\def\vv{\mathbf{v}}
\def\ww{\mathbf{w}}
\def\xx{\mathbf{x}}
\def\yy{\mathbf{y}}
\def\zz{\mathbf{z}}

\def\AA{\mathbf{A}}
\def\BB{\mathbf{B}}
\def\CC{\mathbf{C}}
\def\DD{\mathbf{D}}
\def\EE{\mathbf{E}}
\def\FF{\mathbf{F}}
\def\GG{\mathbf{G}}
\def\HH{\mathbf{H}}
\def\II{\mathbf{I}}
\def\JJ{\mathbf{J}}
\def\KK{\mathbf{K}}
\def\LL{\mathbf{L}}
\def\MM{\mathbf{M}}
\def\NN{\mathbf{N}}
\def\OO{\mathbf{O}}
\def\PP{\mathbf{P}}
\def\QQ{\mathbf{Q}}
\def\RR{\mathbf{R}}
\def\SS{\mathbf{S}}
\def\TT{\mathbf{T}}
\def\UU{\mathbf{U}}
\def\VV{\mathbf{V}}
\def\WW{\mathbf{W}}
\def\XX{\mathbf{X}}
\def\YY{\mathbf{Y}}
\def\ZZ{\mathbf{Z}}

\def\aA{\mathcal{A}}
\def\bB{\mathcal{B}}
\def\cC{\mathcal{C}}
\def\dD{\mathcal{D}}
\def\eE{\mathcal{E}}
\def\fF{\mathcal{F}}
\def\gG{\mathcal{G}}
\def\hH{\mathcal{H}}
\def\iI{\mathcal{I}}
\def\jJ{\mathcal{J}}
\def\kK{\mathcal{K}}
\def\lL{\mathcal{L}}
\def\mM{\mathcal{M}}
\def\nN{\mathcal{N}}
\def\oO{\mathcal{O}}
\def\pP{\mathcal{P}}
\def\qQ{\mathcal{Q}}
\def\rR{\mathcal{R}}
\def\sS{\mathcal{S}}
\def\tT{\mathcal{T}}
\def\uU{\mathcal{U}}
\def\vV{\mathcal{V}}
\def\wW{\mathcal{W}}
\def\xX{\mathcal{X}}
\def\yY{\mathcal{Y}}
\def\zZ{\mathcal{Z}}

\def\Ae{\mathbb{A}}
\def\Be{\mathbb{B}}
\def\Ce{\mathbb{C}}
\def\Le{\mathbb{L}}
\def\Ne{\mathbb{N}}
\def\Pe{\mathbb{P}}
\def\Qe{\mathbb{Q}}
\def\Re{\mathbb{R}}
\def\Se{\mathbb{S}}
\def\Te{\mathbb{T}}
\def\Xe{\mathbb{X}}
\def\Ye{\mathbb{Y}}
\def\Ze{\mathbb{Z}}

\def\btheta{{\bm\theta}}
\def\bzeta{{\bm\zeta}}
\def\bmu{{\bm\mu}}
\def\bZero{\mathbf{0}}
\def\bOne{\mathbf{1}}

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\minimize}{minimize}
\DeclareMathOperator*{\maximize}{minimize}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\rank}{rank}
\DeclareMathOperator{\trace}{tr}
\DeclareMathOperator{\diag}{diag}
\DeclareMathOperator{\diam}{diam}

\def\eps{\varepsilon}
\def\vphi{\varphi}
\def\vsigma{\varsigma}

\def\trans{^{\top}}
\def\deg{^{\circ}}

\def\th{^{\textnormal{th}}}
\def\st{^{\textnormal{st}}}
\def\nd{^{\textnormal{nd}}}
\newcommand\ggreater{\mathbin{>\!\!\!>}}
\newcommand\llesser{\mathbin{<\!\!\!<}}

\newcommand{\YesV}{\ding{51}}%
\newcommand{\NoX}{\ding{55}}%


\DeclareMathSymbol{@}{\mathord}{letters}{"3B}

\newcommand\paren[1]{\left(#1\right)}
\newcommand\abs[1]{\left\lvert#1\right\rvert}
\newcommand\norm[1]{\left\lVert#1\right\rVert}
\newcommand\tuple[1]{\left\langle#1\right\rangle}
\newcommand\inner[2]{\langle #1, #2 \rangle}
\newcommand\timess{\mathbin{\!\times\!}}
\newcommand\nicebar[1]{\mkern 4mu\overline{\mkern-4mu#1}}
\newcommand\ozan[1]{\textcolor{blue}{Ozan says: #1}}
\newcommand\vladlen[1]{\textcolor{red}{Vladlen says: #1}}
\newcommand\creadych[1]{\textcolor{green}{Change in CR: #1}}
\newcommand\creadyadd[1]{\textcolor{cyan}{Add in CR: #1}}
\newcommand\mypara[1]{\vspace{1mm}\noindent\textbf{#1}}
\def\rot#1{\rotatebox{90}{#1}}
\def\latex/{\LaTeX}
\def\bibtex/{\hologo{BibTeX}}
%%%%%%%%%%%%%%%%%%%%%%

==> sections/08_checklist.tex <==
\subsection{Paper Checklist to be included in your paper}

Unless specified otherwise, please answer “yes” to each question if the relevant information is described either in the paper itself or in a technical appendix with an explicit reference from the main paper. If you wish to explain an answer further, please do so in a section titled “Reproducibility Checklist” at the end of the technical appendix.

This paper:
\begin{enumerate}
    \item  Includes a conceptual outline and/or pseudocode description of AI methods introduced (yes/partial/no/NA)
    \answerTODO{yes}
  \item Clearly delineates statements that are opinions, hypothesis, and speculation from objective facts and results (yes/no)
    \answerTODO{yes}
   \item Provides well marked pedagogical references for less-familiare readers to gain background necessary to replicate the paper (yes/no) 
\end{enumerate}




Does this paper make theoretical contributions? \\(yes/no) 
\answerTODO{yes}
\\If yes, please complete the list below.
\begin{enumerate}
  \item All assumptions and restrictions are stated clearly and formally. (yes/partial/no)
    \answerTODO{yes}
  \item All novel claims are stated formally (e.g., in theorem statements). (yes/partial/no)
    \answerTODO{yes}
  \item Proofs of all novel claims are included. (yes/partial/no)
    \answerTODO{yes}
  \item Proof sketches or intuitions are given for complex and/or novel results. (yes/partial/no)
    \answerTODO{yes}
  \item Appropriate citations to theoretical tools used are given. (yes/partial/no)
    \answerTODO{yes}
  \item All theoretical claims are demonstrated empirically to hold. (yes/partial/no/NA)
    \answerTODO{yes}
  \item All experimental code used to eliminate or disprove claims is included. (yes/no/NA)
    \answerTODO{yes}
\end{enumerate}


Does this paper rely on one or more datasets? (yes/no)
    \answerTODO{yes}
\\If yes, please complete the list below.
\begin{enumerate}
  \item A motivation is given for why the experiments are conducted on the selected datasets (yes/partial/no/NA)
    \answerTODO{yes}
  \item All novel datasets introduced in this paper are included in a data appendix. (yes/partial/no/NA)
    \answerTODO{yes}
  \item All novel datasets introduced in this paper will be made publicly available upon publication of the paper with a license that allows free usage for research purposes. (yes/partial/no/NA)
    \answerTODO{yes}
  \item All datasets drawn from the existing literature (potentially including authors’ own previously published work) are accompanied by appropriate citations. (yes/no/NA)
    \answerTODO{yes}
  \item All datasets drawn from the existing literature (potentially including authors’ own previously published work) are publicly available. (yes/partial/no/NA)
    \answerTODO{yes}
  \item All datasets that are not publicly available are described in detail, with explanation why publicly available alternatives are not scientifically satisficing. (yes/partial/no/NA)
    \answerTODO{NA}
\end{enumerate}


Does this paper include computational experiments? (yes/no)
    \answerTODO{yes}
\\If yes, please complete the list below.
\begin{enumerate}
  \item Any code required for pre-processing data is included in the appendix. (yes/partial/no).
    \answerTODO{yes}
  \item All source code required for conducting and analyzing the experiments is included in a code appendix. (yes/partial/no)
    \answerTODO{yes}
  \item All source code required for conducting and analyzing the experiments will be made publicly available upon publication of the paper with a license that allows free usage for research purposes. (yes/partial/no)
    \answerTODO{yes}
  \item All source code implementing new methods have comments detailing the implementation, with references to the paper where each step comes from (yes/partial/no)
    \answerTODO{partial}
 \item If an algorithm depends on randomness, then the method used for setting seeds is described in a way sufficient to allow replication of results. (yes/partial/no/NA)
    \answerTODO{yes}
 \item This paper specifies the computing infrastructure used for running experiments (hardware and software), including GPU/CPU models; amount of memory; operating system; names and versions of relevant software libraries and frameworks. (yes/partial/no)
    \answerTODO{yes}
  \item This paper formally describes evaluation metrics used and explains the motivation for choosing these metrics. (yes/partial/no)
    \answerTODO{yes}
  \item This paper states the number of algorithm runs used to compute each reported result. (yes/no)
    \answerTODO{yes}
  \item Analysis of experiments goes beyond single-dimensional summaries of performance (e.g., average; median) to include measures of variation, confidence, or other distributional information. (yes/no)
    \answerTODO{yes}
  \item The significance of any improvement or decrease in performance is judged using appropriate statistical tests (e.g., Wilcoxon signed-rank). (yes/partial/no)
    \answerTODO{yes}
  \item This paper lists all final (hyper-)parameters used for each model/algorithm in the paper’s experiments. (yes/partial/no/NA)
    \answerTODO{partial}
  \item This paper states the number and range of values tried per (hyper-) parameter during development of the paper, along with the criterion used for selecting the final parameter setting. (yes/partial/no/NA)
    \answerTODO{partial}
\end{enumerate}




\clearpage

